Chemical evolution of galaxies with an environment-dependent stellar initial mass function

The presented study gives a comprehensive overview of the theory and the evidence for a systematically varying stellar initial mass function (IMF). Then we focus on the impact of this paradigm change, that is, from the universal invariant IMF to a variable IMF, on galaxy chemical evolution (GCE) studies. For this aim, we developed the first GCE code, GalIMF, that is able to incorporate the empirically calibrated environment-dependent IMF variation theory, the integrated galactic initial mass function (IGIMF) theory. In this theory, the galaxy-wide IMF is calculated by summing all the IMFs in all embedded star clusters which formed throughout the galaxy in 10 Myr time epochs. The GalIMF code recalculates the galaxy-wide IMF at each time step because the integrated galaxy-wide IMF depends on the galactic star formation rate and metallicity. The resulting galaxy-wide IMF and metal abundance evolve with time. Using this code, we examine the chemical evolution of early-type galaxies (ETGs) from dwarf to the most massive. We find that the introduction of the non-canonical IMF affects the best estimation of the galaxy properties such as their mass, star formation history, and star formation efficiency. Moreover, we are able to provide an independent estimation on the stellar formation timescale of galaxies, the type Ia supernova production efficiency, and constrain the IMF variation law of the low-mass stars. This work provides to the community the publicly available GalIMF code with improved constraints on the IMF variation and has, for the first time, resolved the discrepancy between the galaxy formation timescales obtained from stellar population synthesis and chemical enrichment studies.

==> list_of_publications.tex <==
\section*{List of publications}
\addcontentsline{toc}{section}{List of publications}

This thesis is based on 5 of my first author publications. There are another 4 co-authored publications during my PhD study. The full list of these publications is given below in chronological order.

\begin{enumerate}
%\item Eappen, Kroupa, Wittenburg, \textbf{Yan}, Haslbauer, Jerabkova, and Famaey (2021, in prepare)\\
%“Star-forming timescales in early-type galaxies”
\item \textbf{Yan}, Jeřábková, and Kroupa A\&A, 655, 19 (2021)\\
“Downsizing revised: Longer star formation timescales for elliptical galaxies with an environment-dependent IMF and number of SNIa”
\item Wirth, Jeřábková, \textbf{Yan}, Haas, Šubr, and Kroupa MNRAS, 506, 4131 (2021).\\
“How many explosions does one need? - Quantifying supernovae in globular clusters from iron abundance spreads”
\item \textbf{Yan}, Jeřábková, and Kroupa A\&A, 637, A68 (2020).\\
“Chemical evolution of ultra-faint dwarf galaxies in the self-consistently calculated integrated galactic IMF theory”
\item Chruślińska, Jeřábková, Nelemans, and \textbf{Yan} A\&A, 636, A10 (2020).\\
“The effect of the environment-dependent IMF on the formation and metallicities of stars over the cosmic history”
\item \textbf{Yan}, Jeřábková, and Kroupa A\&A, 632, A110 (2019).\\
“The star formation timescale of elliptical galaxies. Fitting [Mg/Fe] and total metallicity simultaneously”
\item \textbf{Yan}, Jeřábková, Kroupa and Vazdekis A\&A, 629, A93 (2019).\\
“Chemical evolution of elliptical galaxies with a variable IMF. A publicly available code”
\item Jeřábková, Hasani Zonoozi, Kroupa, Beccari, \textbf{Yan}, Vazdekis, and Zhang A\&A, 620, A39 (2018).\\
“Impact of metallicity and star formation rate on the time-dependent, galaxy-wide stellar initial mass function”
\item Kroupa, Jeřábková, Dinnbier, Beccari, and \textbf{Yan} A\&A, 612, A74 (2018).\\
“Evidence for feedback and stellar-dynamically regulated bursty star cluster formation: the case of the Orion Nebula Cluster”
\item \textbf{Yan}, Jeřábková, and Kroupa A\&A, 607, A126 (2017).\\
“The optimally sampled galaxy-wide stellar initial mass function. Observational tests and the publicly available GalIMF code”
\end{enumerate}
